BFAR-Bounded False Alarm Rate detector for improved radar odometry estimation

This paper presents a new detector for filtering noise from true detections in radar data, which improves the state of the art in radar odometry. Scanning Frequency-Modulated Continuous Wave (FMCW) radars can be useful for localization and mapping in low visibility, but return a lot of noise compared to (more commonly used) lidar, which makes the detection task more challenging. Our Bounded False-Alarm Rate (BFAR) detector is different from the classical Constant False-Alarm Rate (CFAR) detector in that it applies an affine transformation on the estimated noise level after which the parameters that minimize the estimation error can be learned. BFAR is an optimized combination between CFAR and fixed-level thresholding. Only a single parameter needs to be learned from a training dataset. We apply BFAR to the use case of radar odometry, and adapt a state-of-the-art odometry pipeline (CFEAR), replacing its original conservative filtering with BFAR. In this way we reduce the state-of-the-art translation/rotation odometry errors from 1.76%/0.5deg/100 m to 1.55%/0.46deg/100 m; an improvement of 12.5%.

==> Scripts/newcommands__functions.tex <==
\newcommand{\ExponentialOf}					[1]	{\mathrm{exp} \left( #1 \right)}
\newcommand{\ConvexHullOf}					[1]	{\mathrm{c.h.} \left( #1 \right)}
\newcommand{\GammaFunctionOf}				[1]	{\Gamma \left( #1 \right)}
\newcommand{\UpperIncompleteGammaFunctionOf}[2]	{\Gamma \left( #1 , #2 \right)}
\newcommand{\LamberWFunction}				[0]	{W}
\newcommand{\LamberWFunctionOf}				[1]	{\LamberWFunction \left( #1 \right)}


\newcommand{\CostFunction}					[0]	{Q}
\newcommand{\CostFunctionOf}				[1]	{\CostFunction \left( #1 \right)}
\newcommand{\CostFunctionOfSensor}			[1]	{\CostFunction_{#1}}
\newcommand{\CostFunctionOfSensorOf}		[2]	{\CostFunctionOfSensor{#1} \left( #2 \right)}




==> Scripts/packages.tex <==
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ %
\usepackage[english]{babel}											%
\usepackage[T1]{fontenc}											%
\usepackage{textcomp}												%
\usepackage{dsfont}													%
\usepackage{booktabs}												%
\usepackage{array}													%
\usepackage{bm}														%
\usepackage{url}													%
\usepackage{enumerate}												%
\usepackage[table]{xcolor}											%
\usepackage{amsmath, amssymb, amsfonts}								% 
\usepackage[section, verbose]{placeins}								%
%\usepackage{subfigure}												%
\usepackage{caption}
\usepackage{subcaption}
\usepackage{cases}													%
\usepackage{ifthen}													%
\usepackage{ifpdf}													%
%\usepackage{enumitem}
\usepackage[pdftex]{graphicx}										% 
\DeclareGraphicsExtensions{.pdf,.png,.jpg,.mps}						%
\pdfminorversion=5													%
%																	%
\usepackage{framed}													%
\usepackage[amsmath,thmmarks,framed,hyperref]{ntheorem}				%
%																	%
\usepackage{eso-pic}												%
\usepackage[switch, pagewise, mathlines]{lineno}					%
\usepackage[color=white!90!black, textwidth=3cm]{todonotes}			%
\usepackage{algorithm}												%
\usepackage[noend]{algpseudocode}									%
\usepackage{acronym}												%
\input{../Scripts/colors}											%
\usepackage{tikz}				% (note: AFTER \pdfminorversion)	%
\usetikzlibrary{calc}												%
%\usetikzlibrary{arrows,decorations.text,decorations.pathmorphing}	%
%\usetikzlibrary{decorations.footprints,fadings,calc,trees,mindmap}	%
\usetikzlibrary{shadows,patterns,positioning,shapes,matrix,fit}		%
%\usetikzlibrary{intersections,plotmarks}							%
\usetikzlibrary{pgfplots.groupplots}
%																	%
% externalization of tikz figures									%
%\usetikzlibrary{external}											%
%\tikzexternalize[shell escape=-enable-write18]						%
%\usepackage[switch, pagewise, mathlines]{lineno}
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ %
%																	%
\usepackage{gensymb}
\usepackage{pgfplots}
%\usetikzlibrary{shapes}												%
%\usetikzlibrary{positioning}
%\usetikzlibrary{fit}
%\usepgfplotslibrary{colormaps}										%
%\usepgfplotslibrary{groupplots}									%
%\pgfplotsset{compat=1.3}											%
%\def\PgfboxplotsWidth{0.5em}										%
%\def\PgfboxplotsOutliersOpacity{0.1}								%
%\input{../Scripts/pgfplots__boxplots_subpackage}					%
%																	%
% to disable ligatures												%
%\usepackage{microtype}												%
%\DisableLigatures{encoding = *, family = *}						%
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ %
\usepackage{color,soul} % for text highlight

\addtolength{\textwidth}{1.0in}
\addtolength{\textheight}{1.00in}
\addtolength{\evensidemargin}{-0.75in}
\addtolength{\oddsidemargin}{-0.75in}
\addtolength{\topmargin}{-.50in}

\theoremstyle{definition} % amsthm only
\newcounter{thm}
\setcounter{thm}{0}
\newtheorem{example}[thm]{Example}



==> Scripts/pgfplots__boxplots_subpackage.tex <==
% files must be of the form:
%
% median     box_top     box_bottom     whisker_top      whisker_bottom

\pgfplotsset{
    box plot/.style={
        /pgfplots/.cd,
        black,
        only marks,
        mark=-,
        mark size=\PgfboxplotsWidth,
        /pgfplots/error bars/.cd,
        y dir=plus,
        y explicit,
    },
    box plot box/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \draw  ##1 -- ++(\PgfboxplotsWidth,0pt) |- ##2 -- ++(-\PgfboxplotsWidth,0pt) |- ##1 -- cycle;
        },
        /pgfplots/table/.cd,
        y index=2,
        y error expr={\thisrowno{3}-\thisrowno{2}},
        /pgfplots/box plot
    },
    box plot top whisker/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark}%
            {\pgfplotserrorbarsmark}%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark options}%
            {\pgfplotserrorbarsmarkopts}%
            \path ##1 -- ##2;
        },
        /pgfplots/table/.cd,
        y index=4,
        y error expr={\thisrowno{2}-\thisrowno{4}},
        /pgfplots/box plot
    },
    box plot bottom whisker/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark}%
            {\pgfplotserrorbarsmark}%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark options}%
            {\pgfplotserrorbarsmarkopts}%
            \path ##1 -- ##2;
        },
        /pgfplots/table/.cd,
        y index=5,
        y error expr={\thisrowno{3}-\thisrowno{5}},
        /pgfplots/box plot
    },
    box plot median/.style={
        /pgfplots/box plot
    },
	box plot outliers/.style={
        /pgfplots/.cd,
        black,
        only marks,
		opacity = \PgfboxplotsOutliersOpacity,
	}
}



